What Matters to You? Towards Visual Representation Alignment for Robot Learning

When operating in service of people, robots need to optimize rewards aligned with end-user preferences. Since robots will rely on raw perceptual inputs like RGB images, their rewards will inevitably use visual representations. Recently there has been excitement in using representations from pre-trained visual models, but key to making these work in robotics is fine-tuning, which is typically done via proxy tasks like dynamics prediction or enforcing temporal cycle-consistency. However, all these proxy tasks bypass the human's input on what matters to them, exacerbating spurious correlations and ultimately leading to robot behaviors that are misaligned with user preferences. In this work, we propose that robots should leverage human feedback to align their visual representations with the end-user and disentangle what matters for the task. We propose Representation-Aligned Preference-based Learning (RAPL), a method for solving the visual representation alignment problem and visual reward learning problem through the lens of preference-based learning and optimal transport. Across experiments in X-MAGICAL and in robotic manipulation, we find that RAPL's reward consistently generates preferred robot behaviors with high sample efficiency, and shows strong zero-shot generalization when the visual representation is learned from a different embodiment than the robot's.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/intro_notes.tex <==
    % \item Vision-based robot learning has made tremendous progress in recent years: given a reward function, robot arms can learn manipulation skills \cite{kalashnikov2018qt, zeng2021transporter, shridhar2022cliport, haldar2023teach}, quadrupeds can gallop through complex terrain \cite{zhuang2023robot, agarwal2023legged}, and articulated hands can perform in-hand rotation \cite{akkaya2019solving, qi2023general}. 
    % and thus should behave in accordance with human preferences. 
    % \item For example, consider a robotic manipulator that is tasked with cleaning your kitchen countertop: there are food scraps that need to be tossed into the trash, and nearby bottles of oil and sauce. Your preferred way to clean up the countertop would be to push the food scraps all-at-once into the trash without knocking over any bottles.
    % \item However, before robots can generate \textit{how} to do the task, they needs to know \textit{what} about the task matters. For example, before the robot can clean a kitchen countertop, it needs to know what cleaning or orderly looks like
    % \item Vision-based robot learning has made tremendous progress in recent years, enabling robots to learn skills which optimize hand-engineered reward functions \cite{}. 
    % \item However, vision-based robot policies will not act in isolation; they will behave around and in service of humans. 
    % \item Here, visual rewards \cite{} have been key in guiding robot behavior during policy optimization, enabling the robot to \abnote{[insert why visual rewards are nice]}. 
    
% \textbf{Pitch-related thoughts.} Context: you have a pre-trained foundation model that understands the visual world, and you want to deploy it on a robot. The challenge: these models pay attention to "everything". Typically, figuring out what is relevant for a particular context is done through task or explicit reward signals. Instead, in this work, we argue that discovering what is relevant for a robot should be personalized and determined by the human end-user. In other words, we ask the question \textit{how can we learn human-centric visual representations for robotics?} 

% \textbf{Pitch Version 0:} Visual foundation models are powerful ways to build image- or video-based representations of the world, and offer promise for robots that act based on visual feedback.
% However, foundation models need to be fine-tuned for downstream robotics tasks.
% Typically, this robot-centric fine-tuning is done through self-supervised task signal (e.g., TCC) or engineered reward signals.
% However, if the robot using such a visual representation should be deployed around and in service of people, then these fine-tuning signals are not guaranteed to capture what matters to the ultimate end-user. In other words, the fine-tuned representations should be personalized for the human. 

% One idea is to fine-tune the robot’s visual representation from human feedback, like preference queries. This has been successful in crowd-sourced large language model alignment [cite].
% However, in the vision-based robotics domain there are two problems: (1) existing preference-based learning is very data inefficient to do for high-dimensional input data like image observations, and (2) SOTA human preference models assume that the person always gives feedback *in-distribution* of the robot embodiment [cite] -- for example, the robot shows the human a screen where the person selects a preferred behavior [cite]; or, the human teleoperates the robot to show what they like and don’t like [cite].

% In contrast, in real-world robotics settings, human feedback can come from more diverse sources of visual data -- a person can do the task on their own to show the robot what they like and what they don’t like. Or, the human can watch another human and express their preferences about the other human’s behavior. Or, the human can indicate which robot behaviors behaviors are aligned with their preferences.
% Inspired by this, our key idea is that human visual representations are *minimally embodiment-dependent*: human visual representations of a task are consistent regardless of if the human is doing the task themselves or if the robot is performing the task.
% If robots can take advantage of this, they can not only scalably fine-tune visual foundation models to be better aligned with human preferences, but they can also optimize for behaviors on their own embodiments which stay in distribution of the human preferences.

% In this work, we contribute:
% \begin{enumerate}
%     \item a unification of fine-tuning visual foundation models for robots
%     \item a new model for fine-tuning visual foundation models from human feedback which is minimally embodiment-dependent
%     \item quantitative experiments showing that our approach is both more data efficient and more robust to OOD data than prior RLHF models (e.g., direct reward prediction) and more aligned with human representations than self-supervised approaches (i.e., TCC).
% \end{enumerate}


\begin{itemize}
    % \item robots that operate on high-dimensional perceptual input like RGB images need to learn how to behave in accordance with human preferences. 
    % \item in the visual robotics domain, by far the most popular way is behavior cloning, which relies on labeled image-action pairs provided by the human to learn a robot policy. While promising, this is bad because this is very sensitive to domain shift and we need huge datasets of demonstrations for every task and every robot. Because you use actions, this also makes the embodiment of the agent super important (e.g., if the robot gets action labels). 
    % \item alternatively, we can try to learn a visual reward function which can be optimized by any robot. Crucial to this reward function is a \textit{representation} of the observations. Prior works have used TCC, MVP, but all
    % \item our idea is to come up with a visual reward that is aligned with the human's representation and incentivizes the robot to generate behaviors that stay in-distribution of the human's representation space. 
    % \item however, how do you know what features matter 
    % \item 
    \item Robots that operate on high-dimensional perceptual input like RGB images need to learn how to behave in accordance with human preferences. 
    \item Visual rewards are important to guide the robot behavior during policy optimization 
    \item Typically the visual rewards are matching the \textit{task} or the \textit{progress} or the \textit{goal} image.
    \item but, what we really want is to have the robot match the \textit{human}'s preference or the human's value. This is beyond notions like progress or goal-matching: e.g., instead of pushing carrots one-by-one, we prefer to group all the carrots together throughout the pushing. Or we prefer the coffee cup to stay away from our valuables like the computer. 
    \item In this work, we argue that if the robot is to optimize for behaviors that are aligned with human values, the robot should understand the visual world the way that the human does. 
    \item We extend the preference-based learning paradigm to the visual robot learning domain by developing a sample-efficient visual reward which captures what the human cares about. 
    \item By optimizing our novel visual reward, the robot is incentivized to stay in-distribution of the visual representation induced by the human teacher. 
    % \item However, we need a visual reward which encodes how the human sees the visual world and stays in-distribution of the representation induced by the 
    % \item To achieve this, our key idea is to 
    % interactively learn a visual representation from human preference feedback that only uses raw observations. and then leverage a visual reward function which encourages the robot to stay in-distribution 
    % \item we want robots to do behaviors in ways that humans like
    % \item if you have "privileged" access to action labels -- e.g., through robot teleoperation -- then life is good. You can match the human's preferred way of doing the task via various methods (e.g., LfD, IL, etc.)
    % \item However, in the real world we do not have actions because its a huge human cost to label actions 
    % \item as vision-based robot policies increasingly operate around and in service of humans, how can we ensure that these high-dim visual policies are aligned with human preferences? 
    % % \item robots will take actions around humans only using raw perceptual input
    % % \item the question is, how can these high-dim visual policies optimize for behaviors that are aligned with the human's preferences? 
    % \item by far the most popular way is to rely on action labels provided by the human to do behavior cloning. This is bad because we need huge datasets of demonstrations for every dataset and every robot. Because you use actions, this makes the embodiment of the agent super important (e.g., if the robot gets action labels). 
    % \item an alternative approach is to learn a reward function which can be optimized by \textit{any} robot. 
    
    % naievly applying this to the visual domain suffers from spurrious correlations and low sample efficiency. 
    % \item alternatively, you can come up with a visual reward which can be optimized by \textit{any} robot. 
    % \item However, this reward function needs to somehow stay in-distribution of the human's preferred behavior. 
    % \item this requires two things: 1) a way to match the behavior and 2) 
    % \item prior works use MVP or TCC to build a visual representation 
    % \item 
    % \item 
    
    % \item 
    % \item in state-space, you can do this via feature matching in IRL or via imitation learning 
    % \item however, if you aren't in state space, and if you are 
    % \item but you 

    % \item when robots are deployed in service of people, they need to perform tasks in ways that humans prefer. 
    % \item this is challenging, because the robot does not know the correct objective function to optimize a priori. This is further complicated because how the human prefers the task done is based on their visual representation, or how they interpret the visual world. 
    % \item Our key idea is the robot's visual reward should incentivize behaviors that are in-distribution of the human's internal representation of the visual world. 
    % \item 
    % \item This raises two natural challenges: 1) in-distribution and 2) preferred representation. 
\end{itemize}



\textbf{Pitch Version 2:}
\begin{itemize}
    \item when robots are deployed around and in service of people, they need to use perceptual sensors like RGB cameras to understand what visual features of the task matter to the end-user. 
    \item For example, consider a robotic manipulator that is tasked with cleaning your kitchen countertop: there are chopped up pieces of onion and carrot, food scraps that need to be tossed into the trash, and nearby bottles of oil and sauce. Your preferred way to clean up the countertop would be to push the food scraps all-at-once into the trash without knocking over any bottles, and rearrange the onion and carrot pieces to be grouped together without touching or mixing. 
    \item In contrast, an \textit{undesirable} way to clean up the countertop involves objects colliding during rearrangement, being manipulated inefficiently (e.g., each scrap is pushed into the trash one-by-one), and the food pieces mixing.
    \item on one hand, the robot could infer the human's preferences by mapping visual observations to a scalar reward. In non-vision-based robotics domains [cite] or in the LLM domain [cite], this is typically done via preference-based learning: the human ranks robot behavior as more or less desirable and the robot infers the associated reward. This is nice because by using human feedback, the robot can hopefully learn the human’s preferred way of doing the task and \textit{implicitly} learn the human's visual features. However, directly learning this mapping from high-dimensional input space like images is (1) data inefficient [cite]and (2) prone to spurious correlations in the implicitly learned representation [cite].
    % \item on the other hand, the robot could focus \textit{explicitly} on learning a visual representation of the task that matches with the visual features that the human cares about. Existing methods for doing this by fine-tuning pre-trained visual representations [cite] task-relevant signals. For example, they assume that the end-user is an expert and can generate expert actions on the robot’s embodiment [cite], or they assume that the robot already knows a good reward function with which it tunes its visual representation of the task [cite]. However, in reality neither of these two visual representation learning methods are realistic for personal robotics: end-users aren't expert teleoperators [cite], and if the robot already knew the right reward that mattered to the end-user, then it could just optimize for it.
    \item in this work, we propose a method to get the best of both worlds: use human feedback to learn the user’s preferred visual representation, and then use this preference-aligned representation for robot behavior generation
    \item specifically, our method utilizes few (i.e., $\leq 30$) video demonstrations of an end-user performing a task in ways consistent with their preferences that are ranked in order of desirability. The preferences expressed in these videos are inherently personalized and go beyond goals: for example, cleaning a countertop includes both pushing food scraps into the trash can \textit{and} avoiding colliding with nearby bottles. Using this insight, we formulate a metric learning problem to infer visual features which disambiguate the preferred and less-preferred human video demonstrations.
    \item using this personalized visual representation, we then enable the robot to optimize behaviors that are consistent with the human’s task preference. Specifically, we take inspiration from optimal transport to design a dense, embodiment-agnostic reward signal that measures the representation alignment between videos induced by the robot and the videos of the end-user used during representation learning.
\end{itemize}



==> sections/sim_environments.tex <==
\subsection{Simulation Environments}
\label{subsec:experiment setup}


\begin{wrapfigure}{r}{0.45\textwidth}
    \vspace{-0.5cm}
    \includegraphics[width=0.45\textwidth]{figs/sim_environments.png}
    \vspace{-0.8cm}
  \caption{X-Magical and IsaacGym tasks.}
  \vspace{-0.5cm}
  \label{fig:x-magical-env}
\end{wrapfigure}

\subsubsection{X-Magical} 
\label{subsubsec:xmagical-setup}
\textbf{Tasks.} We first use the toy simulation environment, X-Magical \citep{zakka2022xirl}. We consider two tasks inspired by kitchen countertop cleaning. The robot always has to push objects to a goal region (e.g., trash can), shown in pink at the top of the scene in \autoref{fig:x-magical-env}. In the \textbf{avoiding} scenario, the end-user prefers that the robot and objects never enter an \textit{off-limits zone} during pushing (blue box in left \autoref{fig:x-magical-env}).
% where the robot needs to push the object (red square) towards a static goal region (light red region) without entering a disfavored region (light blue region). 
In the \textbf{grouping} scenario, the end-user prefers that objects are always pushed \textit{efficiently together} towards the goal region (center, \autoref{fig:x-magical-env}).

\textbf{Privileged State \& Reward.}
For \textbf{avoiding}, the true state $s$ is 7D: planar robot position ($p_\robot \in \mathbb{R}^2$) and orientation ($\theta_\mathrm{R}$),  planar position of the object ($p_{\mathrm{obj}}\in \mathbb{R}^2$), distance between goal region and object, ($d_{\mathrm{obj2goal}}$), and distance between the off-limits zone and the object ($d_{\mathrm{obs2obj}}$). The human's reward is: $\rewh_{\mathrm{avoid}}(s) = - d_{\mathrm{goal2obj}} - 2\cdot \mathbb{I}(d_{\mathrm{obs2obj}} < d_{\mathrm{safety}})$,
For \textbf{grouping}, the state is 9D: $s := (p_\robot, \theta_\robot$, $p_{\mathrm{obj^1}}, p_{\mathrm{obj^2}}, d_{\mathrm{goal2obj^1}}$, $d_{\mathrm{goal2obj^2}})$. The human's reward is: $\rewh_{\mathrm{group}}(s) = - \max(d_{\mathrm{goal2obj^1}}, d_{\mathrm{goal2obj^2}}) - ||p_{\mathrm{obj^1}} - p_{\mathrm{obj^2}}||_2$.
% : $(p_{\mathrm{R}}$, $\theta_\mathrm{R}$, $p_{\mathrm{obj^1}}$, $p_{\mathrm{obj^2}}$, $d_{\mathrm{goal2obj^1}}$ and $d_{\mathrm{goal2obj^2}}$.

% The human's \textbf{avoiding} 
% and for tabletop \textbf{grouping} .

\subsubsection{Robot manipulation} 
\label{subsubsec:manipulation-setup}
\textbf{Task.} We further validate our method in a robot manipulation task in the IsaacGym physics simulator \citep{makoviychuk2021isaac}. We implement the tabletop \textbf{grouping} task, where a robotic arm needs to learn to push two objects \textit{efficiently together} to the end-user's goal region (light blue region in right of \autoref{fig:x-magical-env}). 

\textbf{Privileged State \& Reward.}
The state $s$ is 16D: robot proprioception ($\theta_{\mathrm{joints}}\in \mathbb{R}^{10}$), 3D object positions
($p_{\mathrm{obj^{1,2}}}$), and object distances to goal ($d_{\mathrm{goal2obj^{1,2}}}$). The \textbf{grouping} reward is identical as in Section~\ref{subsubsec:xmagical-setup}. 

